Why Didn't You Listen to Me? Comparing User Control of Human-in-the-Loop Topic Models

To address the lack of comparative evaluation of Human-in-the-Loop Topic Modeling (HLTM) systems, we implement and evaluate three contrasting HLTM modeling approaches using simulation experiments. These approaches extend previously proposed frameworks, including constraints and informed prior-based methods. Users should have a sense of control in HLTM systems, so we propose a control metric to measure whether refinement operations' results match users' expectations. Informed prior-based methods provide better control than constraints, but constraints yield higher quality topics.

==> sections/old.tex <==
% INTRODUCTION

%As a result, it is often necessary to incorporate prior knowledge to improve topic model quality.
%The main intuition behind topic models is that document collections discuss multiple latent topics, where each topic can be represented as a multinomial distribution over a the document collection's vocabulary and each document can be represented as mixture of these latent topics. 
%Latent Dirichlet Allocation (\abr{lda}) \cite{blei2003latent} is one of the most popular topic modeling algorithms, 
%However, often the topics generated by LDA are incomprehensible for humans. \citeauthor{chang2009reading} show that unsupervised topic models may produce incoherent topics because the objective function of topic models may not correlate well with human judgment. Other problems with the generated topics include poorly connected words in topics \cite{mimno2011optimizing}, too many generic words and near duplicate topics \cite{boyd2014care}. Therefore, it is often necessary to incorporate prior knowledge into topic models to improve the quality of the generated topics. 

%Several extensions to LDA add external knowledge for improving topic quality \cite{wallach2006topic, boyd2007topic, chen2013discovering, chen2013leveraging, fan2017prior}. Others propose incorporating human knowledge iteratively during topic model inference \cite{ andrzejewski2009incorporating, hu2014interactive, xie2015incorporating, petterson2010word, pleple2013interactive, smith2018closing}. These iterative methods use feedback provided for a given state of a topic model to guide the modeling process to further improve the topics. We refer to these methods as Human-in-the-loop Topic Modeling (\abr{hltm}) systems. However, it is not  yet understood which of these \abr{hltm} techniques is optimal for supporting users in improving topic models. This paper seeks to provide a comparative framework for determining this.

%\jbgcomment{I think this can be phrased more strongly: Given this panoply of techniques, which is best?  This paper seeks to provide a comparative framework for answering that question.}

%For example, \citeauthor{yang2015efficient} proposed constraint LDA framework and evaluated their system only for word-correlation feedback. 
%\citeauthor{smith2018closing} implemented seven different refinements using informed priors and compared it to a non-interactive system. Such evaluation makes it difficult to 1) understand whether a particular refinement was applied correctly 2) compare their implementation of a particular refinement with other models.   

%\jbgcomment{Please use style checker script and style guide; ``In this work, we'' is redundant.  You can just say ``This paper'' or ``We' \amrcomment{I fixed the specific change; is there a particular script/style guide you're referring to? perhaps in the pinafore directory?  \jbgcomment{https://github.com/Pinafore/pinafore-papers/blob/master/scripts/style-check.rb
%http://www.cs.colorado.edu/~jbg/static/style.html
%}}}

%Although these frameworks provide refinement flexibility, 
%Extending the work of \citeauthor{lee2017human}, we propose a set of nine \textit{user-preferred} refinement operations: add word, change word order, remove word, remove document, add to stop words, create topic, delete topic, merge topics, and split topic.  
%We evaluate for only for a limited set of refinement operations identified by \citeauthor{lee2017human} as those that users wish to use to improve topics.
%We implement these user-preferred refinements across multiple frameworks and compare the resulting implementations using simulations on two datasets. In particular, we implement three systems: (1) Constrained \abr{hltm}, (\textit{const-gibbs}), which is an extension of constrained LDA framework~\cite{yang2015efficient}, (2) informed prior-based, gibbs sampling inference \abr{hltm}, (\textit{info-gibbs}), extending the implementation of~\citeauthor{smith2018closing}, and (3) informed prior-based variational EM inference \abr{hltm}, (\textit{info-vb}).

%We use simulations to compare multiple \abr{hltm} frameworks for a set of nine refinement operations preferred by users \jbgcomment{I'm not sure this is the strongest argument for the set might be worht talking about it a little more (but maybe not in this section)} in prior work~\cite{musialek2016using, lee2017human}.

%add word, change word order, remove word, remove document, add to stop words, create topic, delete topic, merge topics, and split topic. 
%We implement these \textit{user-preferred} refinements for three \abr{hltm} systems that differ in terms of the techniques used for incorporating prior knowledge (informed priors or constraints) and for performing inference (Gibbs sampling or variational). The two systems using Gibbs sampling are direct extensions of prior work~\cite{yang2015efficient, smith2018closing}, but to our knowledge, this paper is the first to implement an \abr{hltm} system using informed priors and variational inference. 


%\jbgcomment{Somewhere, either here or in the next section there needs to be a clearer discussion of what are constraints and priors (now that things are more high level)}

%Prior work in interactive systems underline the importance of providing \textit{control} to end users. Specifically, for \abr{hltm} systems, \citeauthor{smith2018closing} found that users feel frustrated when their refinements are not applied as expected. Current topic model evaluation metrics such as topic coherence, perplexity, and log-likelihood measure the topic model as a whole, and are not sufficient to measure how well a particular refinement is applied. To overcome this issue, we propose an evaluation metric, \textit{control}, which measures how well a \abr{hltm} system incorporates feedback. We use this metric to compare the three \abr{hltm} systems. 

%To compare the \abr{hltm} systems in terms of topic quality improvements and whether they incorporate user feedback as expected (i.e., offer user control), we also introduce new \textit{control} metrics. These metrics should be useful for future evaluations, particularly as prior work has emphasized the importance of providing control to end users of these systems~\cite{smith2018closing}. \jbgcomment{I worry that there are too many self-cites in the introduction that might run afoul of the spirit of anon policy}
%this is the first to propose a metric to explicitly measure how well models incorporate user feedback. 

%Current topic model evaluation metrics such as topic coherence, perplexity, and log-likelihood measure the topic model as a whole, and are not sufficient to measure how well a particular refinement is applied, so we propose a new \textit{control} metric, and use this metric, in addition to topic quality, to compare the three \abr{hltm} systems.

%\jbgcomment{Control is good and important, but can be better phrased.  Talk about ``While previous ITM models talk about the importance of control, this work is the first to create an evaluation to explicitly measure whether\dots''}

% HUMAN FEEDBACK AND LDA

% commenting 2 refinements
% \textbf{Delete topic} In \textit{info-gibbs} and \textit{const-gibbs}, invalidate the topic assignment of all tokens which were previously assigned to $t$. In \textit{info-vb}, remove the row corresponding to $t$ from $\lambda$. Then, for all models, decrease the topic count by 1.

% \textbf{Add to stop words} removes word $w$ from the model. For all three systems, exclude $w$ from the vocabulary, $V$.
%, which removes all occurrences in the corpus.

%\begin{table*}[t!]
%\hline \hline
%\centering
%\begin{tabular}{p{2cm}p{13cm}}
%  Refinement & Implementation details \\
%  \hline \hline
%  Add to stop words & Removes word $w$ from the model. For all three systems, to add $w$ to stop words, exclude $w$ from the vocabulary, $V$. This removes all occurrences in the corpus. \\
%  Remove word & Removes word $w$ from topic $t$. For all three systems, first forget all the word’s tokens $w_i$ from $t$. Then, for \textit{info-gibbs} and \textit{info-vb}, assign a very small prior,\footnote{We use 0.00000001 as $\epsilon$.} $\epsilon$, to $w$ in $t$. For \textit{const-gibbs}, add a constraint\footnote{We use $log(\epsilon)$ to make it a soft constraint. Replacing it with -$\infty$ will make it a hard constraint.} $f_m(z, w, d)$, such that $f_m(z, w, d)=log(\epsilon)$ if $z=t$ and $w=x$, else assign $f_m(z, w, d)= 0$. \\
%  Add word & Adds word $w$ to topic $t$. For all three systems, first forget $w$ from all other topics. Then, for \textit{info-gibbs} and \textit{info-vb}, increase the prior of $w$ in $t$ by the difference between the topic-word counts of $w$ and topic’s top word $\hat{w}$ in $t$. For \textit{const-gibbs}, add a constraint $f_m(z, w, d)$, such that $f_m(z, w, d)$ = 0 if $z=t$ and $w=x$, else assign $f_m(z, w, d) = log(\epsilon)$. \\
%  Remove document & Removes document $d$ from topic $t$. For all models, first forget the topic assignment for all words in the document $d$. Then, for \textit{info-gibbs} and \textit{info-vb}, assign \jbgcomment{Should be clear that this overwrites previous prior value} a very small prior, $\epsilon$, to $t$ in $\alpha_d$. For \textit{const-gibbs}, add a constraint $f_m(z, w, d)$, such that $f_m(z, w, d) = log(\epsilon)$ if $z=t$ and $d=x$, else assign $f_m(z, w, d)=0$.\\
%  Merge topics & Merges topics $t_1$ and $t_2$ into a single topic, $t_1$. For \textit{info-gibbs} and \textit{const-gibbs}, assign $t_1$ to all tokens previously assigned to $t_2$. This effectively removes $t_2$ and updates $t_1$, which should represent both $t_1$ and $t_2$. For \textit{info-vb}, add counts from $\lambda_{t_2}$ to $\lambda_{t_1}$ and remove row from $\lambda$ corresponding to $t_2$.\\
%  Split topic & Splits a topic $t$ given a set of seed words,\jbgcomment{don't use mathmode to spell out words; see Style page} $seed$, into two topics, $t_n$, containing the seed words, and $t$, without the seed words. For each word in the vocabulary, move a fraction of probability mass from parent topic $t$ to $t_n$ as proposed by \cite{pleple2013interactive}. Then, for \textit{info-gibbs} and \textit{info-vb}, assign a high prior\footnote{We use 100 as the high prior. \jbgcomment{I'm worried a little about the selection of these magic numbers; there are a lot of them.  Perhaps would be good to have supplemental file with explanations and justifications}} for all $seed$ in topic $t_n$. For \textit{const-gibbs}, to $seed$ to $t_n$, add a constraint $f_m(z, w, d)$ such that $f_m(z, w, d) = 0$ if $z=t_n$ and $w=w_i \in seed$, else assign $f_m(z, w, d)=log(\epsilon)$.\\
%  Change word order & Rearranges words, such that $w_2$ is higher than $w_1$ in topic $t$. To ensure $w_2$ is ranked higher than $w_1$ in $t$, in \textit{info-gibbs}, increase the prior of $w_2$ in $t$, by the difference between the topic word counts $n_{w_{1,t}}$ -$n_{w_{2,t}}$. In \textit{info-vb}, increase the prior by the difference between  $\lambda_{t,w_1}$ -$\lambda_{t,w_2}$. Intuitively, we supplement counts for word~$w_2$ to rank it higher than word~$w_1$. For \textit{const-gibbs}, compute the ratio~$r$ between the topic word counts' difference $n_{w_{1,t}}$-$n_{w_{2,t}}$ and the counts of word~$w_2$, which have any topic {\bf but}~$t$, $n_{w_{2,x}, x \neq t}$. Then, add a constraint $f_m(z, w, d)$, such that $f_m(z, w, d) = 0$ if $z=t$ and $w=w_2$, else assign $f_m(z, w, d)=\delta$ where $\delta = \log(\epsilon)$ if $r > 1$ else $\delta = 1.0-r$.\\
%  Create topic & Creates a new topic, $t_n$, given a set of seed words, $seed$. First forget the original topic assignment for all seed words, $seed$. Then, for \textit{info-gibbs} and \textit{info-vb}, assign a high prior to $seed$. For \textit{const-gibbs}, to assign $seed$ to $t_n$, add a constraint $f_m(z, w, d)$, such that $f_m(z, w, d) = 0$ if $z=t_n$ and $w=w_i \in seed$, else assign $f_m(z, w, d)=log(\epsilon)$.\\
 % Delete topic & In \textit{info-gibbs} and \textit{const-gibbs}, invalidate the topic assignment of all tokens which were previously assigned to $t$. In \textit{info-vb}, remove the row corresponding to $t$ from $\lambda$. Then, for all models, decrease the topic count by 1.
%\end{tabular}
%\caption{Implementation details for nine \textit{user-preferred refinements}.
%  }
%\end{table*}

%Here we describe implementation details for the nine user-preferred refinements. 
%\begin{enumerate*}
%    \item {\textbf{Add to stop words}}: removes word $w$ from the model. For all three systems, to add $w$ to stop words, exclude $w$ from the vocabulary, $V$. This removes all occurrences in the corpus. 
    
 %    \item{\textbf{Remove word}}: removes word $w$ from topic $t$. For all three systems, first forget all the word’s tokens $w_i$ from $t$. Then, for \textit{info-gibbs} and \textit{info-vb}, assign a very small prior,\footnote{We use 0.00000001 as $\epsilon$.} $\epsilon$, to $w$ in $t$. For \textit{const-gibbs}, add a constraint\footnote{We use $log(\epsilon)$ to make it a soft constraint. Replacing it with -$\infty$ will make it a hard constraint.} $f_m(z, w, d)$, such that $f_m(z, w, d)=log(\epsilon)$ if $z=t$ and $w=x$, else assign $f_m(z, w, d)= 0$.
     
 %  \item {\textbf{Add word}}: adds word $w$ to topic $t$. For all three systems, first forget $w$ from all other topics. Then, for \textit{info-gibbs} and \textit{info-vb}, increase the prior of $w$ in $t$ by the difference between the topic-word counts of $w$ and topic’s top word $\hat{w}$ in $t$. For \textit{const-gibbs}, add a constraint $f_m(z, w, d)$, such that $f_m(z, w, d)$ = 0 if $z=t$ and $w=x$, else assign $f_m(z, w, d) = log(\epsilon)$. 
    
%    \item{\textbf{Remove document}}: removes document $d$ from topic $t$. For all models, first forget the topic assignment for all words in the document $d$. Then, for \textit{info-gibbs} and \textit{info-vb}, assign \jbgcomment{Should be clear that this overwrites previous prior value} a very small prior, $\epsilon$, to $t$ in $\alpha_d$. For \textit{const-gibbs}, add a constraint $f_m(z, w, d)$, such that $f_m(z, w, d) = log(\epsilon)$ if $z=t$ and $d=x$, else assign $f_m(z, w, d)=0$.
    
 %   \item{\textbf{Merge topics}}: merges topics $t_1$ and $t_2$ into a single topic, $t_1$. For \textit{info-gibbs} and \textit{const-gibbs}, assign $t_1$ to all tokens previously assigned to $t_2$. This effectively removes $t_2$ and updates $t_1$, which should represent both $t_1$ and $t_2$. For \textit{info-vb}, add counts from $\lambda_{t_2}$ to $\lambda_{t_1}$ and remove row from $\lambda$ corresponding to $t_2$.
    
%    \item{\textbf{Split topic}}: splits a topic $t$ given a set of seed words,\jbgcomment{don't use mathmode to spell out words; see Style page} $seed$, into two topics, $t_n$, containing the seed words, and $t$, without the seed words. For each word in the vocabulary, move a fraction of probability mass from parent topic $t$ to $t_n$ as proposed by \cite{pleple2013interactive}. Then, for \textit{info-gibbs} and \textit{info-vb}, assign a high prior\footnote{We use 100 as the high prior. \jbgcomment{I'm worried a little about the selection of these magic numbers; there are a lot of them.  Perhaps would be good to have supplemental file with explanations and justifications}} for all $seed$ in topic $t_n$. For \textit{const-gibbs}, to $seed$ to $t_n$, add a constraint $f_m(z, w, d)$ such that $f_m(z, w, d) = 0$ if $z=t_n$ and $w=w_i \in seed$, else assign $f_m(z, w, d)=log(\epsilon)$.
    
%    \item{\textbf{Change word order}}: rearranges words, such that $w_2$ is higher than $w_1$ in topic $t$. To ensure $w_2$ is ranked higher than $w_1$ in $t$, in \textit{info-gibbs}, increase the prior of $w_2$ in $t$, by the difference between the topic word counts $n_{w_{1,t}}$ -$n_{w_{2,t}}$. In \textit{info-vb}, increase the prior by the difference between  $\lambda_{t,w_1}$ -$\lambda_{t,w_2}$. Intuitively, we supplement counts for word~$w_2$ to rank it higher than word~$w_1$. For \textit{const-gibbs}, compute the ratio~$r$ between the topic word counts' difference $n_{w_{1,t}}$-$n_{w_{2,t}}$ and the counts of word~$w_2$, which have any topic {\bf but}~$t$, $n_{w_{2,x}, x \neq t}$. Then, add a constraint $f_m(z, w, d)$, such that $f_m(z, w, d) = 0$ if $z=t$ and $w=w_2$, else assign $f_m(z, w, d)=\delta$ where $\delta = \log(\epsilon)$ if $r > 1$ else $\delta = 1.0-r$. 

 %   \item{\textbf{Create topic}}: creates a new topic, $t_n$, given a set of seed words, $seed$. First forget the original topic assignment for all seed words, $seed$. Then, for \textit{info-gibbs} and \textit{info-vb}, assign a high prior to $seed$. For \textit{const-gibbs}, to assign $seed$ to $t_n$, add a constraint $f_m(z, w, d)$, such that $f_m(z, w, d) = 0$ if $z=t_n$ and $w=w_i \in seed$, else assign $f_m(z, w, d)=log(\epsilon)$.
    
 %   \item{\textbf{Delete topic}}: In \textit{info-gibbs} and \textit{const-gibbs}, invalidate the topic assignment of all tokens which were previously assigned to $t$. In \textit{info-vb}, remove the row corresponding to $t$ from $\lambda$. Then, for all models, decrease the topic count by 1.
%\end{enumerate*}



% SIMULATION METHOD

%To compare the control provided by the different \abr{hltm} systems, we perform a simulation where refinement operations are applied randomly. For each \abr{hltm} system, we first train $20$ LDA models. Then for each refinement, we randomly select a model from the pre-trained models and then apply the refinement. For each refinement, we run $100$ such simulations per \abr{hltm} system. 
%While control metric tells how well a refinement is supported by a \abr{hltm} system, it doesn't provide information about the quality of topics. To estimate the topic quality, we use NPMI~\cite{lau2014machine} topic coherence with wikipedia as a reference corpus. Since randomly applying refinements may worsen the topic quality, we can't use random simulation to estimate the topic quality. To determine that these \abr{hltm} implementations provide an effective way to improve the topic quality, we simulate the behavior of a good user who have access to the document labels and tries to improve topics by intelligently choosing refinement operations. Refer to \ref{sec:appendix} for implementation details of good user.
% Using only 1 dataset to save space
% We use two datasets for our simulation experiments. The first dataset is BBC news \footnote{http://mlg.ucd.ie/datasets/bbc.html}, which includes $2,225$ BBC news articles from the BBC news website corresponding to stories in five different categories (business, entertainment, politics, sports and technology). 
%This dataset contains $500$ articles per category for $14$ different categories (art \& design, business, education, environment, fashion, film, football, law, money, music, politics, science, sports, technology).
%In the first experiment, we apply refinements randomly. 
%This is unlikely to improve topic quality, so this experiment focuses on measuring the \textit{control} provided by the \abr{hltm} systems. 
%For the second experiment, we simulate the behavior of a good user who has access to document labels and intelligently chooses the refinement operations to improve the topic quality. Please refer to appendix \ref{sec:appendix} for good user simulation details. Here \lkfcomment{``here'' meaning for only GOOD user? if so why not do this for random user too??} we measure \textit{control} as well as the final model's topic coherence using NPMI\cite{lau2014machine} with Wikipedia as the reference corpus. 

\begin{figure*}
\includegraphics[scale=0.65]{sections/figures/gnews_random_user.pdf}
\caption{\textit{control} score for the three systems and seven refinements for the ``random user''. Each refinement operation is selected randomly 100 times.}
\label{fig:random_user}
\end{figure*}

\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
 & \multicolumn{3}{l|}{const-gibbs} & \multicolumn{3}{l|}{info-gibbs} & \multicolumn{3}{l|}{info-vb} & \multicolumn{3}{l|}{Kruskal Wallis} \\ 
 \hline
 & Mean & Median & SD & Mean & Median & SD & Mean & Median & SD & $\chi^2$ & df & p \\ \hline
Add word & 0.82 & 0.91  & 0.29 & 1.0 & 1.0 & 0 & 0.98 & 0.99 & 0.04 &  &  & 0 \\ \hline
Change word order & 0.41 & 0.35 & 0.53 & 1.19& 	1.06 & 0.46 & 1.02 & 1 & 0.27 &  &  & \\ \hline
Create topic & 0.079 & 0 & 0.10 & 0.98 & 1&	0.11 &1  &1  &0  &  &  & \\ \hline
Merge topic & 0.97 & 1 & 0.05 & 0.96 & 1 & 	0.05& 0.99 & 1 & 0.02 &  &  &\\ \hline
Remove document & 1 & 1 & 0 & 1 & 1 & 0 & 0.72& 	1 &	0.39 &  &  &\\ \hline
Remove word & 1 & 1 & 0 & 1 & 1 & 0 & 1 & 1 & 0 &  &  &  \\ \hline
Split topic & 0.91 &0.92 & 0.09 & 0.93 & 	0.93 & 0.06 & 1 & 1 & 0 &  &  &\\ \hline

\end{tabular}
\caption{\textit{control} score for the three systems and seven refinements for the ``random user''. Each refinement operation is selected randomly 100 times.}
\label{table:random_user}
\end{table*}

\subsection{Simulation Results}
\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
\hline
 & \multicolumn{3}{l|}{const-gibbs} & \multicolumn{3}{l|}{info-gibbs} & \multicolumn{3}{l|}{info-vb}  \\ 
 \hline
 & Random & \multicolumn{2}{l|}{Good} & Random & \multicolumn{2}{l|}{Good} & Random & \multicolumn{2}{l|}{Good} \\ 
 \hline
 & Control & Control & Quality-3 & Control & Control & Quality-3 & Control & Control & Quality-3 \\
 \hline
Add W & .82, .29 & .86, .24 & 0.30, *  & 1.0, 0.0 & .98, .03 & .31, * & .98, .04 & .67, .39 & .17, * \\ \hline
Reorder W & 0.41, 0.53 & * & 0.16, * & 1.19, 0.46 & * & -0.01, * & 1.02, 0.27 & * & -0.01, * \\ \hline
Create T & 0.08, 0.10 & * & -0.66, * & 0.98, 0.11 & * & -1.1, * & 1.0, 0.0 & * & -1.3, * \\ \hline
Merge T & 0.97, 0.05 & * & 0.63, * & 0.96, 0.05 & * & -0.04, * & 0.99, 0.02 & * & 0.14, * \\ \hline
Remove D & 1.0, 0.0 & * & -0.17, * & 1.0, 0.0 & * & 0.08, * & 0.72. 0.39 & * & -0.60, * \\ \hline
Remove W & 1.0, 0.0 & * & 0.54, * & 1.0, 0.0 & * & 0.30, * & 1.0, 0.0 & * & 0.12, * \\ \hline
Split T & 0.91, 0.09 & * & 0.19, * & 0.93, 0.06 &  * & -0.79, * & 1.0, 0.0 & * & -0.16, *\\ \hline

\end{tabular}
\caption{\textit{control} scores for the three \abr{hltm} systems and the seven refinements for both simulated users. Coherence deltas reported for only the ``good user''. Scores reported as (mean, SD)}
\label{table:random_user}
\end{table*}
